Temporal Model Adaptation for Person Re-Identification

Person re-identification is an open and challenging problem in computer vision. Majority of the efforts have been spent either to design the best feature representation or to learn the optimal matching metric. Most approaches have neglected the problem of adapting the selected features or the learned model over time. To address such a problem, we propose a temporal model adaptation scheme with human in the loop. We first introduce a similarity-dissimilarity learning method which can be trained in an incremental fashion by means of a stochastic alternating directions methods of multipliers optimization procedure. Then, to achieve temporal adaptation with limited human effort, we exploit a graph-based approach to present the user only the most informative probe-gallery matches that should be used to update the model. Results on three datasets have shown that our approach performs on par or even better than state-of-the-art approaches while reducing the manual pairwise labeling effort by about 80%.

==> algo/accsvrg.tex <==
\begin{algorithm}[t]
\scriptsize
 \SetKwInput{KwSet}{Set}
 \SetKwRepeat{KwRepeat}{Repeat}{Until}
 \SetKwFor{KwIterate}{Iterate}{}{}
 \KwIn{$\learningrate > 0$, $\batchsize > 0$, $\nesterovpar > 0$ $\kernellowrankapprox^{(1)}$,$\metriclowrankapprox^{(1)}$,$\featpairstrainingset$}
 \KwIterate{$s=1, 2, \ldots$ }
 {
	\uline{1. Compute the full gradients for all training samples using the current epoch optimal solutions}
	\\
	\algoindent
	$\grad{\lossfun_{\kernellowrankapproxepoch}} = \frac{1}{n} \sum_{i=1}^{n} \grad{\hinge_{\kernellowrankapproxepoch}(\pairi)}$
	, \quad
	$\grad{\lossfun_{\metriclowrankapproxepoch}} = \frac{1}{n} \sum_{i=1}^{n} \grad{\hinge_{\metriclowrankapproxepoch}(\pairi)}$
		
	\uline{2. Set}
	\\
	\algoindent		
	$\kernellowrankbatchapprox^{(1)} = \kernellowrankapproxepoch$
	, \quad
	$\metriclowrankbatchapprox^{(1)} = \metriclowrankapproxepoch$
		
	\KwIterate{$t=1, \ldots, K$}
	{
		\uline{1. Uniformly sample $\batchsize$ pairs from the training set $\featpairstrainingset$}
		\\
		\algoindent
		$\minibatchset^{(t)} = \{\featpair^{(j)} \}_{j=1}^{m}$
		\\
		\uline{2. Compute the mini-batch gradients as in eq.(\ref{eq:mini_batch_gradient})}
		\\
		\algoindent
		$\grad{\lossfun_{\kernellowrankbatchapproxiter}^{\minibatchset}} =  \frac{1}{\batchsize}\sum_{j=1}^{\batchsize} \grad{ \hinge_{\kernellowrankbatchapproxiter}(\pairj) } - \frac{1}{\batchsize}\sum_{j=1}^{\batchsize}\grad{\hinge_{\kernellowrankapproxepoch}(\pairj) } + \grad{\lossfun_{\kernellowrankapproxepoch}}$
		\\
		\algoindent
		$\grad{\lossfun_{\metriclowrankbatchapproxiter}^{\minibatchset}} =  \frac{1}{\batchsize}\sum_{j=1}^{\batchsize} \grad{ \hinge_{\metriclowrankbatchapproxiter}(\pairj) } - \frac{1}{\batchsize}\sum_{j=1}^{\batchsize}\grad{\hinge_{\metriclowrankapproxepoch}(\pairj) } + \grad{\lossfun_{\metriclowrankapproxepoch}}$
		\\
		\uline{3. Compute the proximal mappings using the current optimal mini-batch solutions and the mini-batch gradients}
		\\
		\algoindent
		$\kernellowrankbatchapproxiterupd = \proxoperator(\kernellowrankbatchapproxiter - \learningrate \grad{\lossfun_{\kernellowrankbatchapproxiter}^{\minibatchset}} )$
		, \quad
		$\metriclowrankbatchapproxiterupd = \proxoperator(\metriclowrankbatchapproxiter - \learningrate \grad{\lossfun_{\metriclowrankbatchapproxiter}^{\minibatchset}} )$
		\\
		\uline{4. Apply Nesterov acceleration}
		\\
		\algoindent
		$\kernellowrankbatchapproxiterupd = \kernellowrankbatchapproxiterupd + \nesterovpar(\kernellowrankbatchapproxiterupd-\kernellowrankbatchapproxiter)$
		\\
		\algoindent
		$\metriclowrankbatchapproxiterupd = \metriclowrankbatchapproxiterupd + \nesterovpar(\metriclowrankbatchapproxiterupd-\metriclowrankbatchapproxiter)$	   
	}
	
	\uline{3. Update the optimal solutions}
	\\
	\algoindent
	$\kernellowrankapproxepochupd = \kernellowrankbatchapprox^{(K)}$
	,
	\quad
	$\metriclowrankapproxepochupd = \metriclowrankbatchapprox^{(K)}$
	
 }
 \caption{Accelerated Stochastic Low-Rank Sparse Dissimilarity-Similarity Learning}
 \label{algo:accsvrg}
\end{algorithm}

==> algo/sadmm.tex <==
\begin{algorithm}[t]
\scriptsize
 \SetKwInput{KwSet}{Set}
 \SetKwRepeat{KwRepeat}{Repeat}{Until}
 \SetKwFor{KwIterate}{Iterate}{}{}
 \KwIn{$\learningrate > 0$, $\admmpenalty > 0$, $S>0$ $\kernellowrank^{(1)}$,$\metriclowrank^{(1)}$,$\featpairstrainingset$}
 \KwIterate{$s=1, \ldots, S$ }
 {
	\uline{1. Compute the full partial derivatives using all training samples}
	\\
	 \algoindent
	 $\pder{}{\kernellowrankepoch}\lossfun_{\kernellowrankepoch,\metriclowrankepoch} = \frac{1}{n}\sum_{i=1}^{n} \pder{}{\kernellowrankepoch}\hinge_{\kernellowrankepoch,\metriclowrankepoch}(\pairi)$
	 \\
	 \algoindent
	  $\pder{}{\metriclowrankepoch}\lossfun_{\kernellowrankepoch,\metriclowrankepoch} = \frac{1}{n}\sum_{i=1}^{n} \pder{}{\metriclowrankepoch}\hinge_{\kernellowrankepoch,\metriclowrankepoch}(\pairi)$
		
	\uline{2. Set}
	\\
	\algoindent		
	$\kernellowrankapprox^{(1)} = \kernellowrankepoch$
	, \quad
	$\metriclowrankapprox^{(1)} = \metriclowrankepoch$
		
	\KwIterate{$t=1, \ldots, n$}
	{
		\uline{1. Update $\kernellowrankapproxiter$}
		\\
		\algoindent
		$\kernellowrankapproxiterupd = \kernellowrankapproxiter - \learningrate \Biggl( \pder{}{\kernellowrankapproxiter}\hinge_{\kernellowrankapproxiter,\metriclowrankapproxiter}(\pairiter) - \pder{}{\kernellowrankepoch}\hinge_{\kernellowrankepoch,\metriclowrankepoch}(\pairiter)$
		\\
		\algoindent \hspace{10em} $+ \pder{}{\kernellowrankepoch}\lossfun_{\kernellowrankepoch,\metriclowrankepoch} + \admmpenalty \left(\kernellowrankapproxiter - \kernellowranklagrepoch + \kernellowranklagrmultepoch/\admmpenalty\right)  \Biggr)$
		\\ 
		\uline{2. Update $\metriclowrankapproxiter$}
		\\
		\algoindent $\metriclowrankapproxiterupd = \metriclowrankapproxiter - \learningrate \Biggl( \pder{}{\metriclowrankapproxiter}\hinge_{\kernellowrankapproxiterupd,\metriclowrankapproxiter}(\pairiter) - \pder{}{\metriclowrankepoch}\hinge_{\kernellowrankepoch,\metriclowrankepoch}(\pairiter)$
		\\
		\algoindent \hspace{10em} $+  \pder{}{\metriclowrankepoch}\lossfun_{\kernellowrankepoch,\metriclowrankepoch} + \admmpenalty \left(\metriclowrankapproxiter - \metriclowranklagrepoch + \metriclowranklagrmultepoch/\admmpenalty\right)\Biggr)$   
	}
	
	\uline{3. Update $\kernellowrankepoch$ and $\metriclowrankepoch$}
	\\
	\algoindent
	$\kernellowrankepochupd = \frac{1}{n}\sum_{t=1}^{n}\kernellowrankapproxiter$
	\\
	\algoindent
	$\metriclowrankepochupd = \frac{1}{n}\sum_{t=1}^{n}\metriclowrankapproxiter$
			
	
	\uline{4. Update $\kernellowranklagrepoch$ and $\metriclowranklagrepoch$}
	\\
	\algoindent
	$\kernellowranklagrepochupd = \left( \kernellowrankepochupd_{i,:}+\kernellowranklagrmultepoch_{i,:}/\admmpenalty \right)\max\left(0, 1- \frac{\kernellowrankpar}{ \admmpenalty \norm{\kernellowrankepochupd_{i,:}+\kernellowranklagrmultepoch_{i,:}/\admmpenalty}_2} \right)$
	\\
	\algoindent
	$\metriclowranklagrepochupd = \left( \metriclowrankepochupd_{i,:}+\metriclowranklagrmultepoch_{i,:}/\admmpenalty \right)\max\left(0, 1- \frac{\metriclowrankpar}{ \admmpenalty \norm{\metriclowrankepochupd_{i,:}+\metriclowranklagrmultepoch_{i,:}/\admmpenalty}_2} \right)$
	
	\uline{5. Update $\kernellowranklagrmultepoch$ and $\metriclowranklagrmultepoch$}
	\\
	\algoindent
	$\kernellowranklagrmultepochupd = \kernellowranklagrmultepoch + \admmpenalty \left( \kernellowrankepochupd- \kernellowranklagrepochupd \right)$
	\\
	\algoindent
	$\metriclowranklagrmultepochupd = \metriclowranklagrmultepoch + \admmpenalty \left( \metriclowrankepochupd- \metriclowranklagrepochupd\right)$
 }
 \KwOut{Estimated optimal solutions
 %$\kernellowrank = \frac{1}{S}\sum_{s=1}^{S}\kernellowrankepoch$
 $\kernellowrank = \kernellowrank^{(S)}$
 and 
  %$\metriclowrank = \frac{1}{S}\sum_{s=1}^{S}\metriclowrankepoch$
  $\metriclowrank = \metriclowrank^{(S)}$
 }
 \caption{Stochastic ADMM optimization for Low-Rank Sparse Similarity-Dissimilarity Learning}
 \label{algo:sadmm}
\end{algorithm}

==> tables/3DPeS.tex <==
\begin{table}
	\scriptsize
	\centering
	\caption{Comparison with state-of-the-art methods on the 3DPeS dataset.
	 Best results for each rank are in boldface font.}
    \label{tab:3DPeS_Comparison}
    \begin{tabulary}{1\linewidth}{L{10em}||C{4em}|C{4em}|C{4em}|C{4em}||C{4em}||L{10em}}
	\toprule
    Rank $\rightarrow$   & 1  & 5 & 10 & 20 & Labeled [\%] & Reference \tabularnewline
	\midrule
	CSL				& \textbf{57.9}	& \textbf{81.1}	& \textbf{89.5}	& 93.7	& 100	& ICCV 2015~\cite{Shen2015} \\
	$\myalgoname_4^{\mathrm{MS}}$ & 57.25 & 76.75 & 86.45 & \textbf{95.83} & 19.06	& Proposed \\
	kLFDA			& 54.0	& 77.7	& 85.9	& 92.4	& 100	& ECCV 2014~\cite{Xiong2014} \\
	KEPLER			& 51.37	& 76.18 & 84.32	& 92.13	& 100	& TIP 2015~\cite{Martinel2015c} \\
	$\myalgoname_0$	& 47.91 & 76.03 & 85.54 & 92.51 & 100	& Proposed \\
	$\myalgoname_4$	& 47.52 & 75.67 & 84.96 & 92.14 & 22.31	& Proposed \\
	rPCCA			& 47.3	& 75.0	& 84.5	& 91.9	& 100	& ECCV 2014~\cite{Xiong2014} \\	
	$\myalgoname_3$	& 44.75 & 69.76 & 82.50 & 93.75 & 16.18	& Proposed \\
	$\myalgoname_2$	& 41.67 & 65.62 & 80.21 & 85.42 & 10.48	& Proposed \\
	%SWF        	& 40.74 & 64.84	& 73.58 & 82.74	& 100 & ECCV 2014~\cite{Martinel2014b}    \\   
	%LED   			& 35.35 & -		& 73.91 & 82.61 & 100 & SPL 2015~\cite{Martinel2014b}    \\
	IMS-LFDA    	& 38.71 & 61.64	& 72.22 & 82.54 & 100   & CVPR 2015~\cite{Li2015}         \\
	$\myalgoname_1$	& 38.02 & 53.54 & 62.08 & 75.62 & 5.25 & Proposed \\
	LFDA			& 34.24	& 59.31	& 70.13	& 81.12	& 100	& CVPR 2013~\cite{Pedagadi2013}			\\
	KISSME 			& 32.76 & 57.65	& 68.51	& 79.71	& 100	& CVPR 2012~\cite{Kostinger2012}	\\
	PRDC			& 34.04	& 57.74	& 64.37 & 73.84	& 100	& TPAMI 2013~\cite{Zheng2012a}		\\
	eSDC			& 27.25	& 56.16	& 66.82 & 74.88	& 100	& CVPR 2013~\cite{Zhao2013}		\\	
	\bottomrule
    \end{tabulary}
\end{table}


==> tables/CUHK02_P1.tex <==
\begin{table}[t]
\scriptsize
\centering
\caption{Comparison with state-of-the-art methods on the CUHK Campus dataset.
	    Results for existing methods have been computed using a multiple-shot strategy. Results for our approach are given for both the single shot ($\myalgoname^{1}$) and multiple-shot ($\myalgoname^{2}$)
	    Best results are in boldface font.}
\label{tab:CUHK02_comparison} 
	\begin{tabulary}{1\linewidth}{L{7em}||C{3em}|C{3em}|C{3em}|C{3em}|C{3em}|C{3em}||C{5.5em}||L{9em}}
	\toprule
    Rank $\rightarrow$   & 1  & 5 & 10 & 20 & 50 & 100 & Labeled [\%] & Reference \\
	\midrule
	MLAPG & 64.24 & \NA & 90.84 & 94.92 & \NA & \NA & 100 & ICCV2015~\cite{Liao2015a} \\
	XQDA  & 63.21 & \NA & 90.04 & 94.16 & \NA & \NA & 100 & CVPR2015~\cite{Liao2015} \\
	$\myalgoname_4$  	& 42.47 & 62.68 & 72.58 & 81.86 & 93.40 & 97.53 & 24.25 & Proposed \\
	$\myalgoname_3$  	& 42.47 & 62.68 & 72.58 & 81.86 & 93.40 & 97.53 & 24.25 & Proposed \\
	$\myalgoname_2$  	& 42.47 & 62.68 & 72.58 & 81.86 & 93.40 & 97.53 & 24.25 & Proposed \\
	$\myalgoname_1$  	& 42.47 & 62.68 & 72.58 & 81.86 & 93.40 & 97.53 & 24.25 & Proposed \\
	KEPLER 			& 38.85 & 65.28 & 76.12 & 84.72 & 92.85 & 96.58 & 100 & TIP2015~\cite{Martinel2015c}\\
	LMF 			& 34.30 & 55.21 & 64.96 & 74.94 & \NA & \NA & 100 & CVPR 2014~\cite{Zhao2014} \\
	SalMatch		& 28.45 & 45.85 & 55.67 & 67.95 & 84.52 & 92.26 & 100 & ICCV2013~\cite{Zhao2013a}	\\
	PatMatch		& 20.39 & 34.12 & 41.09 & 51.56 & 72.46 & 87.91 & 100 & ICCV2013~\cite{Zhao2013a}	\\	    
	%TML(Our\_Generic) & 20.53 & 45.54 & 56.61 & 69.62 & 85.74 & 93.75 & 100 & ACCV2012~\cite{Li2012a}	\\
	\bottomrule
    \end{tabulary}   
%    \vspaceaftertable
\end{table}

==> tables/CUHK03.tex <==
\begin{table}[t]
\scriptsize
	\centering
	 \caption{Rank 1 performance comparison with state-of-the-art methods on the CUHK03 dataset.
	 Best results are in boldface font.}
   	\label{tab:CUHK03_comparison}
   	\begin{tabulary}{1\linewidth}{L{10em}||C{7em}|C{7em}||C{7em}||L{10em}}
	\toprule
				    & Labeled & Detected & Labeled [\%] & Reference \\ 
	\midrule   
	%LRME 			& 62.1	& \NA	& 100 & CVPR 2015~\cite{Paisitkriangkrai2015} \\
	MLAPG			& \textbf{57.96} & \textbf{51.15} & 100 & ICCV 2015~\cite{Liao2015a} \\ 
	$\myalgoname_4$	& 54.78 & 48.13 & 19.09/21.41 & Proposed \\
	IDLA			& 54.74	& 44.96 & 100 & CVPR 2015~\cite{Ahmed2015} \\
	XQDA			& 52.20 & 46.25 & 100 & CVPR 2015~\cite{Liao2015} \\ 
	$\myalgoname_3$	& 50.64 & 44.23 & 13.59/17.12 & Proposed \\
	$\myalgoname_2$	& 44.12 & 37.74 & 10.43/11.21 & Proposed \\
	$\myalgoname_1$	& 35.98 & 32.51 & 6.11/6.11 & Proposed \\		
	DRSCH-128		& 21.96	& \NA 	& 100 & TIP 2015~\cite{Zhang2015} \\
	DeepReID		& 20.65 & 19.89	& 100 & CVPR 2014~\cite{Li2014} 	\\
	DRSCH-64		& 18.74	& \NA 	& 100 & TIP 2015~\cite{Zhang2015} \\
	KISSME 			& 14.17 & 11.70 & 100 & CVPR 2012~\cite{Kostinger2012} \\
	%LDML 			& 13.51 & 10.92 & 100 & ICCV 2009~\cite{Guillaumin2009} \\
	\bottomrule	
	\end{tabulary}
	\vspaceaftertable
%	\vspace{-1em}
\end{table}

==> tables/GRID_distractors.tex <==
\begin{table}
	\centering
	 \caption{Comparison with state-of-the-art methods on the GRID dataset.
 Best results for each rank are in boldface font.}
   	\label{tab:GRID_comparison_distractors}
   	\begin{tabulary}{1\linewidth}{L{8.5em}||C{3em}|C{3em}|C{3em}|C{3em}|C{3em}||L{8em}}
	\toprule
    Rank $\rightarrow$   & 1  & 5 & 10 & 15 & 20 & Publication \\
	\midrule
	KEPLER			& 18.40 & 39.12 & 50.24 & 57.04 & 61.44 & TIP 2015~\cite{Martinel2015c} \\
	MLAPG			& 16.64 & 41.20 & 52.96 & \NA	& \NA   & ICCV 2015~\cite{Liao2015a} \\
	XQDA 			& 16.56 & 33.84 & 41.84 & 47.68 & 52.40 & CVPR 2015~\cite{Liao2015} \\ 
	PKFM			& 16.3	& 35.8	& 46.0	& 52.8	& 57.6	& CVPR 2015~\cite{Chen2015} \\
	MtMCML			& 14.08 & 34.64 & 45.84 & 52.88 & 59.84 & TIP 2014~\cite{Ma2014a} \\ 
	MRank-RankSVM   & 12.24 & 27.84 & 36.32 & 42.24 & 46.56 & ICIP 2013~\cite{Loy2013} \\ 
	MRank-PRDC      & 11.12 & 26.08 & 35.76 & 41.76 & 46.56 & ICIP 2013~\cite{Loy2013}\\ 
	PRDC			& 9.68  & 22.00 & 32.96 & 38.96 & 44.32 & TPAMI 2012~\cite{Zheng2012a}\\ 
	\bottomrule
   	\end{tabulary}
\end{table}
